The Challenge of the EMC Effect: existing data and future directions

Since the discovery that the ratio of inclusive charged lepton (per-nucleon) cross sections from a nucleus A to the deuteron is not unity - even in deep inelastic scattering kinematics - a great deal of experimental and theoretical effort has gone into understanding the phenomenon. The EMC effect, as it is now known, shows that even in the most extreme kinematic conditions the effects of the nucleon being bound in a nucleus can not be ignored. In this paper we collect the most precise data available for various nuclear to deuteron ratios, as well as provide a commentary on the current status of the theoretical understanding of this thirty year old effect.

==> texfiles/theory-old.tex <==
\section{Status of Theory}
%
The challenge of understanding the EMC effect~\cite{Aubert:1983xm} from a theoretical perspective has forced nuclear physicists to confront questions at the very heart of nuclear physics; namely, how do nuclei emerge from QCD and are there ascertainable remnants of this emergence in nuclear structure? After the more than 30 years since the discovery of the EMC effect the implications of QCD for nuclear structure are far from understood.

The immediate parton model interpretation of the EMC effect
is that the valence quarks inside a nucleus carry a smaller fraction of momentum than the valence quarks inside a free nucleon. The question remains however, what is the mechanism that causes this redistribution of quark momenta? Numerous explanations of the EMC effect have been proposed, e.g., nuclear binding~\cite{Akulinichev:1985ij,Akulinichev:1985xq,Akulinichev:1986gt,Akulinichev:1990su,Dunne:1985ks,Dunne:1985cn,Bickerstaff:1989ch,Benhar:1997vy}, pion excess in nuclei~\cite{Ericson:1983um,Berger:1983jk,Berger:1984na,Berger:1987er,Bickerstaff:1989ch}, multi-quark clusters~\cite{Jaffe:1982rr,Carlson:1983fs,Chemtob:1983zj,Clark:1985qu,Miller:1985un}, dynamical rescaling~\cite{Nachtmann:1983py,Close:1983tn}, medium modification~\cite{Bentz:2001vc,Mineo:2003vc,Smith:2003hu,Cloet:2005rt,Cloet:2006bq,Cloet:2009qs,Cloet:2012td} and short-range correlations~\cite{Weinstein:2010rt,Arrington:2012ax,Frankfurt:2012qs,Hen:2012fm,Hen:2013oha}.
This section will canvas some of the more prominent ideas put forward to explain the EMC effect over the last several decades, before doing so however, we will briefly discuss a few salient aspects of DIS on nuclear targets which are pertinent to the EMC effect.

DIS on nuclear targets is potentially a rich area of experimental research that remains largely unexplored. For example, a nuclear target with total angular momentum $J$ has $2\,J+1$ independent structure functions in the Bjorken limit~\cite{Jaffe:1988up,Cloet:2006bq}, and thus far only the spin-averaged $F_2(x_A)$ structure function has been measured for nuclei with $A > 3$. Progress is being made however, with the HERMES data~\cite{Airapetian:2005cb} for the deuteron $b_1(x)$ structure function\footnote{An interpretation of the HERMES data, relevant to understanding the EMC effect, can be found in, e.g., Ref.~[\refcite{Miller:2013hla}].} and further measurements planned at Jefferson Lab~\cite{Chen:2011aa}. Measurement of the $2\,J+1$ structure functions for $A > 3$ nuclei, while challenging, could shed important light on the role of QCD in nuclear structure.

From a QCD perspective the various nuclei are bound states of an infinite number of quarks and gluons, defined by their valence quark content and discrete quantum numbers, in direct analogy to hadrons. The empirical fact that the valence quark content of nuclei can be replaced by their nucleon content in the classification of nuclei is already strong evidence for what may be called traditional nuclear physics, where the quarks and gluons of QCD are completely frozen inside the hadronic nuclear constituents and play no direct role in nuclear structure. In this picture QCD is of little relevance to nuclear structure beyond the nucleon--nucleon potential and the various hadronic matrix elements, e.g., nucleon form factors and parton distributions.

To confront that EMC effect theoretically one must determine the quark distributions of nuclei, which for quarks of flavor $q$ are defined by
%
\begin{align}
q_{A}\left(x_A\right) &= \int\frac{d\xi^-}{2\pi} e^{iP^+\,x_A\,\xi^-/A}
\left< A,P \left| \overline{\psi}_q(0)\,\gamma^+\,\psi_q(\xi^-)\right| A,P \right>,
\label{eq:nuclearpdf}
\end{align}
%
where $A$ labels the nucleus, $P$ its 4-momentum, $\psi_q$ is a quark field of flavor $q$ and $x_A$ is the Bjorken scaling variable.\footnote{The nuclear structure functions or quark distributions are often defined per-nucleon, in that case Eq.~\eqref{eq:nuclearpdf} and its corollaries would have an extra factor of $A^{-1}$.} 
In theoretical calculations it is customary to define the Bjorken scaling variable for a nuclear target as
%
\begin{align}
x_A \equiv A\,\frac{Q^2}{2\,P\cdot q} = A\,\frac{Q^2}{2\,M_A\,\nu} =  \frac{Q^2}{2\,\bar{M}_N\,\nu}
=  x_p\, \frac{M_p}{\bar{M}_N},
\label{eq:bjorkenxA}
\end{align}
%
where $A$ is the nucleon number, $q$ is the momentum transfer, $M_A$ is the mass of the nucleus,  $\bar{M}_N \equiv M_A/A$, $M_p$ is the proton mass and $x_p$ is the familiar scaling variable for the proton. The quark distributions (and structure functions) therefore have support on the domain $0 < x_A < A$. Note, in DIS experiments on nuclear targets the experimental structure functions are usually extracted from data as a function of the Bjorken scaling variable for the proton, $x_p$, therefore when comparing theory with experiment Eq.~\eqref{eq:bjorkenxA} should be used to replace $x_A$ with $x_p$~\cite{Hen:2013oha}.

For any explanation of the EMC effect to be credible the baryon number and momentum sum rules must remain satisfied, which for nuclear targets take the form:
%
\begin{align}
\label{eq:sumrulesbaryon}
&\int_0^A dx_A\, u_A^-(x_A) = 2\,Z + N, \hspace{5mm}
\int_0^A dx_A\, d_A^-(x_A) = Z + 2\,N,  \\
% 
\label{eq:sumrulesmomentum}
&\int_0^A dx_A\, x_A\left[u_A^+(x_A) + d_A^+(x_A) + \ldots + g_A(x_A)\right] = Z + N = A,
\end{align}
%
where $Z$ and $N$ are the proton and neutron number, respectively; $g_A(x_A)$ is the nuclear gluon distribution function; and the plus and minus type quark distributions are defined by $q^{\pm}(x) = q(x) \pm \bar{q}(x)$.

All proposed explanations for the EMC effect discussed in the following sections provide a qualitative description of the data, at least in the region usually associated with the EMC effect, that is, $0.3 \lesssim x_A \lesssim 0.7$. Therefore an ability to distinguish between many of these various mechanisms will only be possible with new experiments that probe genuinely novel aspects of nuclear PDFs, important examples are their flavor dependence and spin structure. These new directions will be discussed from an experimental standpoint in Sect.~\ref{sec:future}, however in this section we will endeavor to highlight how this next generation of EMC type measurements will help to distinguish between the various mechanisms thought responsible for the EMC effect.


%===============================================================================
%===============================================================================
\subsection{Traditional Convolution Models}
%
From a traditional nuclear physics perspective it is natural to think of DIS on nuclear targets as a two step process; the virtual photon first scatters from a quark confined inside a hadronic nuclear constituent, giving the PDFs of the bound hadron; these PDFs are then combined with the lightcone distribution of the struck hadron inside the nucleus.
%where these hadronic constituents are then distributed inside the nucleus. 
The total result giving the PDFs of the nuclear target. This process is illustrated in Fig.~\ref{fig:convolution}a and assumes an incoherent sum over the hadronic constituents; this formalism is often called the convolution model and ignores, e.g., the interaction of the structure hadron with the nuclear remnant as depicted in Figs.~\ref{fig:convolution}b and \ref{fig:convolution}c, which illustrate, respectively, gluon and quark exchange processes~\cite{Hoodbhoy:1986fn}.

The nuclear PDFs of Eq.~\eqref{eq:nuclearpdf} are represented in the convolution formalism by:
%
\begin{align}
q_{A}\left(x_A\right) &= \sum_{\alpha} \int_0^A dy_A \int_0^1 dz\ \delta\!\left(x_A - y_A\,z\right)\ f^{\alpha}_A(y_A)\ q_{\alpha}(z),
\label{eq:convolution}
\end{align}
%
where $\alpha$ is a sum over the hadronic nuclear constituents, e.g., nucleons, pions, deltas, etc. The quark distributions inside the bound hadrons $q_{\alpha}(z)$ are assumed to equal those of their free counterparts and $f^{\alpha}_A(y_A)$ is the lightcone momentum distribution (Fermi smearing function) of a hadron $\alpha$ in the nuclear target, which, in analogy to Eq.~\eqref{eq:nuclearpdf} has the formal definition
%
\begin{align}
f_{A}\left(y_A\right) &= \int\frac{d\xi^-}{2\pi} e^{iP^+\,y_A\,\xi^-/A}
\left< A,P \left| \overline{\psi}_\alpha(0)\,\gamma^+\,\psi_\alpha(\xi^-)\right| A,P \right>.
\label{eq:}
\end{align}
%
The scaling variable is given by $y_A = A\,\frac{p^+}{P^+}$ where $p^+$ is the plus-component of momentum for the bound hadron. For the baryon number and momentum sum rules of Eqs.~\eqref{eq:sumrulesbaryon} and \eqref{eq:sumrulesmomentum} to hold in the convolution framework, the Fermi smearing functions must satisfy
%
\begin{align}
\sum_{\alpha} \int_0^A dy_A\, f^{\alpha}_A(y_A) &= A, 
&
\sum_{\alpha} \int_0^A dy_A\, y_A \, f^{\alpha}_A(y_A) &= A.
\label{eq:fermisumrules}
\end{align}
%
What surprised many with the discovery of the EMC effect was that if the nucleus is assumed to consist only of nucleons ($\alpha = \text{protons}, \text{neutrons}$) then there exists no reasonable choice for $f^{p,n}_A(y_A)$ that can explain the EMC data~\cite{Miller:2001tg}. This observation changed our understanding of nuclear structure and its relation to QCD, because, prior to the discovery of the EMC effect, it was thought by many that quark and gluon degrees of freedom, characterized by the scale $\Lambda_{\text{QCD}} \simeq 250\,$MeV, would be unaffected by nuclear structure, which is typified by binding energies of $\sim\!10\,$MeV per-nucleon.

%===============================================================================
\begin{figure}[tbp]
\centering\includegraphics[width=\columnwidth,clip=true,angle=0]{figures/convolution_model}
\caption{Diagram (a) is a representation of the convolution formalism, where the virtual photon interacts with a quark confined inside a bound hadron. In the traditional convolution formalism diagrams of the type depicted in (b) and (c) are ignored, therefore the remnant of the struck hadron does not feel the nucleon medium during the interaction with the virtual photon. This is not the case in explanations of the EMC effect based on medium modification, which are discussed in Sect.~\ref{sec:medium_modification}. Diagrams like those illustrated in (b) and (c) do not vanish in the Bjorken limit~\cite{Jaffe:1985je}.}
\label{fig:convolution}
\end{figure}
%===============================================================================

In nuclear structure pions are responsible for, \textit{inter alia}, the long range part of the nucleon--nucleon interaction, it is therefore natural to include pions in the sum of Eq.~\eqref{eq:convolution}. This idea implies an excess of pions in nuclei when compared to the free nucleon, and was one of the first explanations of the EMC effect~\cite{Ericson:1983um,Berger:1983jk,Berger:1984na,Berger:1987er,Bickerstaff:1989ch} grounded in traditional nuclear physics. The lightcone distribution of pions inside the nucleus $f^{\pi}_A(y_A)$ should peak at $y_A \sim m_\pi/\bar{M}_N$, whereas $f^{p,n}_A(y_A)$ has its peak at $y_A \sim 1$, therefore the introduction of pions into the convolution model shifts momentum from the valence quark region to the region where $x_A \lesssim 0.2$. In Ref.~[\refcite{Berger:1983jk}], for example, it was demonstrated that if pions carry 5\% of the nuclear lightcone momentum -- corresponding to an extra 0.13 pions per-nucleon -- then the qualitative features of the EMC effect in iron could be explained. An immediate consequence of the pion excess model is the prediction that there should be a significant enhancement of the sea-quark distributions in nuclei, however, as discussed in Sect.~IV the pion Drell-Yan experiments~\cite{Alde:1990im} at Fermilab in the late 1980s, and later charged pion electroproduction experiments at Jefferson Lab~\cite{Gaskell:2001fn,Gaskell:2001xr}, found no such enhancement, leading some authors to ask the question: where are the nuclear pions?\cite{Bertsch:1993vx} 
%Including delta baryons in Eq.~\eqref{eq:convolution} may alleviate this discrepancy somewhat, however the delta PDFs are completely unknown.

The role of nuclear pions could potentially be clarified via measurements of the EMC effect in the spin-dependent structure function $g_{1A}$ (see Eq.~\eqref{eq:pemc} for a definition of the polarized EMC effect). Pions are spin zero and therefore the spin-dependent lightcone momentum distribution of pions inside a nucleus, $\Delta f^{\pi}_A(y_A)$, vanishes. A consequence therefore is that a naive pion excess model, based on Eq.~\eqref{eq:convolution}, should predict that the EMC effect in polarized structure functions would be much smaller than the original EMC effect, this is on contrast to the dynamical rescaling and medium modification approaches discussed in the following two sections.


%===============================================================================
%===============================================================================
\subsection{Dynamical rescaling}
%
Almost immediately after the discovery of the EMC effect it was observed that the per-nucleon $F_{2A}(x,Q^2)$ structure function of iron resembles the nucleon structure function $F_{2N}(x,Q^2)$, only at a larger value of $Q^2$, that is
%
\begin{align}
F_{2A}(x,Q^2) \simeq F_{2N}(x,\,\xi_A(Q^2)\,Q^2),
\label{eq:dynamical_rescaling}
\end{align}
%
where the rescaling factor satisfies $\xi_A(Q^2) > 1$. The properties of DGLAP evolution then produces the required quenching of the nuclear structure functions in the valence quark region but also a significant enhancement for $x \lesssim 0.1$, which, while seen in the original EMC data, disappeared in subsequent experiments.

This dynamical rescaling behavior was attributed to an increase in the confinement radius for quarks inside bound nucleons, as compared to their free counterparts; a consequence of the closely backed neighboring nucleons whose wave functions are often overlapping. A physical motivation for Eq.~\eqref{eq:dynamical_rescaling} can be obtained by noting that a factorization scale $\mu^2$ is associated with PDFs, which separates perturbative from nonperturbative physics. In perturbative QCD $\mu^2$ also provides an infrared cutoff for radiative gluons, therefore, an increased confinement radius for quarks inside bound nucleons implies $\mu_A^2 < \mu_N^2$. Assuming 
%
\begin{align}
q_A(x,Q^2=\mu_A^2) = q_N(x,Q^2=\mu_N^2),
\end{align}
%
leading-order DGLAP evolution then implies Eq.~\eqref{eq:dynamical_rescaling} where 
%
\begin{align}
\xi_A(Q^2) = \left[\frac{\mu_N^2}{\mu_A^2}\right]^{\alpha_s(\mu_N^2)/\alpha_s(Q^2)}.
\end{align}
%
If the confinement and factorization scales are related by
%
\begin{align}
\frac{r_A}{r_N} = \frac{\mu_N}{\mu_A},
\end{align}
%
then the value of $\xi \simeq 2$ at $Q^2 = 20\,$GeV$^2$ needed to qualitatively explain the EMC effect implies an increase in the confinement radius of about 15\%.

For polarized nuclear structure functions dynamical rescaling would predict a polarized EMC effect of a comparable size to the usual unpolarized EMC effect, therefore polarized DIS experiments on nuclear targets could help disentangle dynamical rescaling from alternative explanations of the EMC effect, like pion excess.


%===============================================================================
%===============================================================================
\subsection{Medium Modification \label{sec:medium_modification}}
%
The successes of more than 60 years of traditional nuclear physics teaches us that nuclei are composed largely of color single objects whose properties closely resemble those of free nucleons. These nucleons bound inside the nucleus are separated by distance scales similar to their actual size; as a consequence the wave functions of the bound nucleons are often overlapping. From a QCD perspective this could result in, e.g, quark exchange between nucleons~\cite{Hoodbhoy:1986fn} or the formation of hidden color configurations~\cite{Miller:2013hla}. It is therefore natural to conclude that the internal structure of all bound nucleons could be modified -- with respect to their free counterparts -- by the presence of the nuclear medium. This is known as medium modification. 

Aspects of medium modification are present in dynamical rescaling, associated with the change in confinement radius, however this idea was put on a firmer footing with the development of the quark-meson-coupling (QMC) model~\cite{Guichon:1987jp,Guichon:1995ue,Saito:2005rv}. In the QMC model nuclei are composed of bound nucleons
described by MIT bags, which are bound together by the exchange of mesons between the quarks of nearby nucleons. In its simplest form the model consists of an isoscalar--scalar ($\sigma$) and an isoscalar--vector ($\omega$) mean-field which self-consistently couples to the quarks inside the bound nucleons, causing a change in their internal quark structure. This model provides a self-consistent quark level description of the nuclear medium, giving the correct saturation properties of nuclear matter, and effective Skyrme forces in good agreement with other contemporary studies~\cite{Dutra:2012mb}.

%===============================================================================
\begin{figure}[tbp]
\subfloat{\centering\includegraphics[width=0.48\columnwidth,clip=true,angle=0]{figures/EMCs_nuclearmatter_v2}}
\subfloat{\centering\includegraphics[width=0.48\columnwidth,clip=true,angle=0]{figures/EMC_effects_lead_anl}}
\caption{\textit{Left panel}: Results for the EMC (solid line) and polarized EMC (dashed line) effects in  nuclear matter from Refs.~[\protect\refcite{Cloet:2005rt,Cloet:2006bq}]. 
\textit{Right panel}: EMC effect (solid line) for nuclear matter with a $Z/N$ ratio equal to lead and this result split into quark flavors. The data in both figures is taken 
from Ref.~[\protect\refcite{Sick:1992pw}].}
\label{fig:emc_effects}
\end{figure}
%===============================================================================

The MIT bag model does not provide a covariant description of nucleon structure. This shortcoming has been addressed in Refs.~[\refcite{Bentz:2001vc,Mineo:2003vc,Cloet:2005rt,Cloet:2006bq,Cloet:2009qs,Cloet:2012td}] where a quark-level description for atomic nuclei has been constructed using the Nambu--Jona-Lasinio (NJL) model. This framework is similar in spirit to the QMC model in that the mean scalar and vector fields couple to the quarks inside the bound hadrons, thereby self-consistently modifying their quark structure. This model gives excellent results for the nucleon structure functions~\cite{Cloet:2005pp,Cloet:2007em} and provides a natural explanation for the EMC effect; the result for symmetric nuclear matter is illustrated as the solid line in the left panel of Fig.~\ref{fig:emc_effects}.
In this approach the EMC effect arises from an interplay between the mean scalar and vector fields in the nuclear medium. The scalar field reduces the dressed quark mass in-medium, $M^* < M$, which also reduces the nucleon mass, this tends to shift the nuclear PDFs to larger $x$ relative to the free nucleon. The mean vector field shifts the energy of all quarks in the medium, which produces a scale transform for a bound nucleon PDF given by
%
\begin{align}
q(x) &= \frac{p^+}{p^+ - V^+}\ \tilde{q}\left(\frac{p^+}{p^+ - V^+}\,x - \frac{V_q^+}{p^+ - V^+}\right),
\end{align}
%
where $\tilde{q}(x)$ is the nucleon PDF without the effect of the vector field, $p^+$ is the nucleon plus-component of momentum and $V^+$ is the plus-component of the mean vector field. The Fermi motion of the bound nucleons is included in a manner similar to Eq.~\eqref{eq:convolution}, except the sum is now over medium modified nucleons. The combination of these effects gives the results in Fig.~\ref{fig:emc_effects}.

This approach has also made predictions for the EMC effect in the spin-dependent nuclear structure function $g_{1A}(x_A)$. The polarized EMC effect can be defined by~\cite{Cloet:2005rt,Cloet:2006bq}
%
\begin{align}
\Delta R_{\text{EMC}} =\frac{g_{1A}}{g^{\text{naive}}_{1A}}
=\frac{g_{1A}}{P^{A}_{p}\,g_{1p} + P^{A}_{n}\,g_{1n}},
\label{eq:pemc}
\end{align}
%
where $g_{1p}$ and $g_{1n}$ are the free nucleon structure functions and $P^{A}_{p(n)}$ is the polarization of the protons (neutrons) in the nucleus $A$. The result for the polarized EMC effect -- for a polarized proton embedded in nuclear matter -- is given by the dashed line in the left panel of Fig.~\ref{fig:emc_effects}. The polarized EMC effect is found to be twice that of the usual EMC effect. A mean-field calculation using the chiral soliton model~\cite{Smith:2005ra} found a polarized EMC effect of comparable size to the spin-averaged EMC effect. The differences between the two models is attributed to the inclusion of antiquarks in the chiral soliton model. In these models the large polarized EMC effect is caused by a dramatic enhancement in the lower components of the quark wave functions in medium, which converts quark spin to quark orbital angular momentum.

This quark-level description of nuclei based on the NJL model has also made predictions for flavor dependence of the EMC effect for $N \neq Z$ nuclei~\cite{Cloet:2009qs,Cloet:2012td}. Predictions for this flavor dependence in nuclear matter with a $Z/N$ ratio equal to that of lead are illustrated in Figs.~\ref{fig:emc_effects}. In these calculations -- for $N>Z$ nuclei -- the isovector-vector mean field increases the binding of the $u$ quarks and decreases the binding for the $d$ quarks, which results in a significant flavor dependence for the EMC effect.

%===============================================================================
%===============================================================================
\subsection{Short-Range Correlations and Multi-quark Clusters}
%
The EMC effect originates because of the multiple nucleons that constitute nuclei; it is therefore natural to attempt to understand the EMC effect through features of the nucleon-nucleon potential. Sect.~3 introduced the recent observations of a series of papers~\cite{Weinstein:2010rt,Arrington:2012ax,Frankfurt:2012qs,Hen:2012fm,Hen:2013oha} which point out the strong linear correlation between the height of the $x_p > 1$  plateaus observed in inclusive quasi-elastic electron scattering and the slope of the EMC effect, for a large set of nuclear targets. The observed plateaus in the range $1.5 \lesssim x_p \lesssim  2.0$ are attributed to two-nucleon short-range correlations (SRCs) in the nuclear wave function. SRCs are characterized by high relative but low center-of-mass momentum, in comparison to the Fermi momentum, which is typically $k_F \simeq 200-270\,$MeV. Modern nuclear wave functions, e.g., determined using Green's function or variational Monte Carlo techniques, tend to have large high momentum components~\cite{Wiringa:2013ala}. For example, the momentum distributions of Ref.~[\refcite{Wiringa:2013ala}] give a probability of $\sim\!13\,$--$20$\% for a given nucleon to have a momentum greater than $270\,$MeV for nuclei with $4 \leqslant A \leqslant 12$. Detailed results are given in Tab.~\ref{tab:kf_probabilities}.

%===============================================================================
\begin{table}[b]
%\addtolength{\extrarowheight}{2.2pt}
\addtolength{\tabcolsep}{5.0pt}
\centering
\tbl{Percentage probability that a proton or neutron will have a momentum greater than $270\,$MeV for various $A \leqslant 12$ nuclei; calculated from the momentum distributions of Ref.~[\protect\refcite{Wiringa:2013ala}].} 
{\begin{tabular}{l|cccccccc}
\hline\hline
             & ${}^2$H & ${}^3$H  & ${}^3$He & ${}^4$He & ${}^7$Li & ${}^9$Be & ${}^{11}$B & ${}^{12}$C  \\
\hline
proton (\%)  & 4.3     & 5.8      & 9.0      & 12.9    & 12.2     & 13.5     & 15.6     & 19.5    \\
neutron (\%) & 4.3     & 9.2      & 5.7      & 12.9    & 10.3     & 11.8     & 14.6     & 19.5    \\
\hline\hline
\end{tabular}}
\label{tab:kf_probabilities}
\end{table}
%===============================================================================

Explanations of the EMC effect based on SRCs also rely on the medium modification of the bound nucleon wave function~\cite{Sargsian:2012sm,Hen:2013oha}, where the degree of modification is proportional to the virtuality, $v = p^2 - M^2$, of the bound nucleon. In the previous section -- where the medium modification is induced by the mean fields -- each bound nucleon is modified at the level of a few percent, if medium modification is caused by SRCs then an explanation of the EMC effect requires modifications many times larger (because far fewer nucleons undergo modification). With existing data it is not possible to distinguish between mean-field induced medium modification and that associated with SRCs~\cite{Hen:2013oha}. 

Knockout reactions have found that SRCs between $pn$ pairs are about a factor $20$ more likely than $pp$ or $nn$ SRCs. For $N > Z$ nuclei protons are therefore more likely to be associated with SRCs in the nuclear wave function. The SRC explanation of the EMC effect then implies that bound protons undergo larger medium modification than neutrons in nuclei with $N > Z$~\cite{Sargsian:2012sm}, such as lead. Therefore, since $u$ quarks dominate the proton, the up quark distribution in $N > Z$ nuclei should have a larger EMC effect than the down quark distribution. This flavor dependence of the EMC effect is similar to that induced by an isovector--vector mean field discussed in the previous section. As such, measurements of the flavor dependence of the EMC effect are unlikely to distinguish between the mean-field and SRC mechanisms. Measurements of the polarized EMC effect may however help unravel these two effects. For example, the proton spin contributes approximately $87$\%~\cite{Wiringa:2013ala} of the total angular momentum for the ${}^7$Li nucleus and of this $87$\% only $2.6$\% is from nucleons with momentum above $270\,$MeV; which is a factor $4$ less than the spin-averaged case (see Tab.~\ref{tab:kf_probabilities}). Mean-field induced medium modification produces an EMC effect and polarized EMC effect of comparable size for ${}^7$Li~\cite{Cloet:2006bq}, for SRCs to produce a similar result the medium modification of the bound $g_{1p}$ structure function must be $4$ times that for the spin averaged structure. Therefore, compared with mean-field induced medium modifications, comparable polarized and spin-averaged EMC effects require SRC induced medium modifications in spin structure functions approximately $20$ times larger than the mean-field approach. Therefore, comparable polarized and spin-averaged EMC effects appears less likely if SRCs are the mechanism responsible.

Two medium modification mechanisms that fit naturally with SRCs is quark exchange between nucleons~\cite{Hoodbhoy:1986fn} and the formation of multiquark ($6,\,9,\,12,\ldots$) clusters~\cite{Jaffe:1982rr,Carlson:1983fs,Chemtob:1983zj,Clark:1985qu,Miller:1985un}. Both these ideas have been extensively discussed since the discovery of the EMC effect. In Ref.~[\refcite{Hoodbhoy:1986fn}] it was demonstrated that quark exchange between overlapping nucleons may explain a substantial portion of the EMC effect. Multiquark clusters shift valence quark momenta to $x_A > 1$, momentum conservation then demands a depletion in the EMC region. To explain the EMC effect in iron a six-quark bag probability of $20$--$30$\% is needed~\cite{Carlson:1983fs,Miller:1985un}, which is consistent with the probability of high momentum protons or neutrons in iron~\cite{Sargsian:2012sm}.

The slope of the EMC effect is not only correlated with the SRC plateaus, in  Refs.~[\refcite{Benhar:2012nj,Arrington:2012ax}] it was pointed out that there also exits a strong linear correlation with the mean removal energy for nucleons in nuclei. The mean removal energy is sensitive to the global properties of the nuclear wave function, not just the short distance piece associated with SRCs. In Refs.~[\refcite{Benhar:2012nj,Arrington:2012ax}] the mean removal energy was determined using the Koltun sum rule~\cite{Koltun:1974zz} with various approximations for the nuclear spectral functions. Although a correlation exists, direct calculations of the EMC effect incorporating these type of binding effects are generally thought to not fully explain the EMC effect~\cite{Hen:2013oha}.





